Dataplant: Enhancing System Security with Low-Cost In-DRAM Value Generation Primitives

DRAM manufacturers have been prioritizing memory capacity, yield, and bandwidth for years, while trying to keep the design complexity as simple as possible. DRAM chips do not carry out any computation or other important functions, such as security. Processors implement most of the existing security mechanisms that protect the system against security threats, because 1) executing security mechanisms usually require non-trivial computational capabilities (e.g., encryption), and 2) commodity DRAM chips are not designed to perform computations or tasks other than data storage. In this work, we advocate for DRAM as a key component for providing security mechanisms to the system. To this end, we propose Dataplant, a new class of low-cost, high-performance, and reliable security primitives that can be integrated in commodity DRAM chips with minimal changes. The main idea of Dataplant is to slightly modify the internal DRAM timing signals to expose the inherent process variation found in all DRAM chips for generating unpredictable but reproducible values (e.g., keys) within DRAM. We use Dataplant to build two new security mechanisms. First, a new Dataplant-based physical unclonable function (PUF) with non-destructive read-out, low evaluation latency, robust responses, resiliency to temperature changes, and data-independent responses. Second, a new cold boot attack prevention mechanism that automatically destroys all data within DRAM on every power cycle with zero run-time energy and latency overheads. Using a combination of detailed simulations and experiments with 136 real commodity DRAM chips, we show that our Dataplant-based PUF has 1.8x higher throughput than the best state-of-the-art DRAM PUFs. We also demonstrate that our Dataplant-based cold boot attack protection mechanism is 19.5x faster and consumes 2.54x less energy when compared to existing mechanisms.

==> EntropySeeds.tex <==
%!TEX root =  main.tex
\subsection{Generating High-Entropy Numbers}
\label{sec:seeds}

Truly random numbers are important for many security protocols. Public-key encryption schemes use random numbers to achieve security, key exchange
algorithms use random numbers to establish secret session keys, and commitment schemes use random numbers to hide committed values~\cite{Corrigan-Gibbs:2013}. The security of these schemes relies heavily on the unpredictability of the random input values. Hence when the inputs are not truly random the security of the system breaks down~\cite{corriganrecommendations,  CVE-2001-0950,CVE-2001-1141,CVE-2001-1467,CVE-2003-1376,CVE-2005-3087,CVE-2006-1378,CVE-2006-1833,CVE-2007-2453,CVE-2008-0141,CVE-2008-0166,CVE-2008-2108,CVE-2008-5162,CVE-2009-3238,CVE-2009-3278,CVE-2011-3599,lenstra2012ron,Yilek:2009,heninger2012mining,costin2014large}.

Lack of entropy sources in IoT devices is a major problem, making diverse and scary attacks possible across the internet~\cite{heninger2012mining, costin2014large}. The main reason is, again, the low cost nature \changes{of} the hardware used in these devices. \mechanism can help with this problem by using its \uesa{} and \upla{} for generating high-entropy random numbers that can be used directly or as seeds to securely bootstrap other pseudo-random number generators. We evaluate the quality of these random numbers in Section~\ref{sec:nist}.


==> applications.tex <==
%!TEX root =  main.tex

%\section{Security Mechanisms}
%\label{sec:apps}

%We now discuss four important security mechanisms that \mechanism enables for low-cost devices:
%(1)~authentication with PUFs,
%(2)~preventing cool boot attacks,
%(3)~low-cost secure deallocation for reducing the lifetime of critical data. 

\input{051_PUFs}
\input{052_coldBootAttacks}
%\input{otherMechanisms}
%\input{EntropySeeds}
%\input{secureDeallocation} 


==> otherMechanisms.tex <==
%!TEX root =  main.tex

\section{Other Security Mechanisms \\ Enabled by \mechanism }
%\section{Other Dataplant Applications}

\label{sec:othermechanisms}

\mechanism{} enables the implementation of a variety of applications in the security domain. We already describe two important applications enabled by \mechanism{}, authentication mechanisms based on PUFs and preventing cold boot attacks. In this section we briefly discuss an additional application that can be implemented with \mechanism{}.

%\subsection{Secure Memory Deallocation}
\vspace{3pt}\noindent\textbf{Secure Memory Deallocation.}
\label{sec:early_destruction}
Today's applications, especially web servers, web browsers, and word processors, do not immediately remove data from memory when it is no longer needed. Instead, the data is physically erased only when the memory is required for other uses. As a consequence, sensitive data could remain in memory for an indefinite amount of time, which augments the risk of exposure.

Secure deallocation~\cite{chow2005shredding, Anikeev:2013, Sha2018, harrison2007protecting, geambasu2009vanish, Garfinkel:2004} is a technique that set the data to zero at the moment of deallocation, or as soon as the data is not needed anymore. This technique reduces the time that critical data is exposed to attacks. Vanish~\cite{Geambasu2009} propose a similar idea in which the old copies of data are self-destroyed after a specific amount of time.

\mechanism{} enables the implementation of the previous techniques with very low latency, energy, and area overhead. We evaluate a \mechanism-based secure deallocation mechanism that incurs only an 0.8\%/0.6\% penalty on performance/energy compared to a system without secure deallocation, and using a variety of applications. We evaluate our \mechanism-based secure deallocation mechanism in Appendix~\ref{sec:eval_dealloc}. 

%For lack of space, we will include our through evaluation in an extended version of the paper.

%\subsection{Accelerating Page Allocations}
%\label{sec:initialization}
%\label{sec:pagealloc}

%The OS has the responsibility of mapping the virtual addresses to physical addresses, manage page faults, etc. But it also has the responsibility of destroying previous data in new mapped pages, as otherwise, the information would leak between processes. The Linux kernel achieves this by zeroing the pages before the first access from the application. Zeroing pages can have a significant performance overhead~\cite{valat2013introducing}. We can perform memory zeroing efficiently with our D-TRAN implementation (Section~\ref{sec:d-tran}). The method is as simple as emitting a \mechanism{} to the targeted row when a page initialization is performed.

%Rowclone~\cite{seshadri2013} and Lisa-clone~\cite{Chang2016LISA} had proposed in-DRAM methods to initialize data to zero by copying a reserved row filled with zeros, to the destination row. These solutions need to modify the internal architecture of DRAM and the capacity of the DRAM is slightly reduced. Our \mechanism{} does not have these problems,  and the hardware overhead, energy, latency and the complexity of \mechanism{} is lower.











































%In addition to preventing cold boot attacks, our \mechanism{} could be beneficial for other applications in the security domain. In this section, we explain a few of them (Sections~\ref{sec:physicallyUnclonable}, \ref{sec:pagealloc} and \ref{sec:early_destruction}). We also describe the additional changes in the system required to implement the applications described in this section and other applications which require controlling \mechanism{} by software (Section~\ref{sec:implications}).

%\subsection{Physically Unclonable Functions (PUFs)}
%\label{sec:physicallyUnclonable}
%%\todo{write it better}

%Physically unclonable functions (PUFs)~\cite{Gassend:2002, Daihyun2005, Suh2007, Maes2010, Tehranipoor:2015} rely on process variation to generate a chip's unique identifier (UID) as a digest of its physical peculiarities. As a consequence, PUFs are commonly used as a low-cost authentication mechanism~\cite{Maes2010}.%\ipnote{By definition PUFs are not used to generate random numbers in a classical sense. But if you want we can keep this by saying that in most cases (probably including ours) this comes as a nice side property} or for generating random, but reproducible, cryptographic keys. %Furthermore, they can be used as random numbers generators for getting encryption keys.

%PUFs' inputs are usually referred to as challenges and their outputs as responses~\cite{Maes2010}. Among the properties desired for a PUF, the response for a given challenge should be different and randomly distributed on different devices. However, under the same conditions\footnote{These conditions are generally difficult to ensure, as they might include factors such as: random noise, temperature of operation, and supply voltage, to name a few.} %To account for said environment variations, the hamming distance of two responses for the same challenge on the same device is limited to a max amount.}
%, the same device should produce the same response when given the same challenge.

%% Our Approach does not need to disable the refresh.

%%The goal of a PUF is to generate both UIDs and random numbers.

%%As explained in Section~\ref{sec:u-esa} and Section~\ref{sec:u-pla}, the values produced by U-ESA and U-PLA depend on the sense amplifier's (SA) process variation, but also on the SA's design.
%As explained in Section~\ref{sec:u-esa} and Section~\ref{sec:u-pla}, U-ESA and U-PLA can generate some unpredictable values which depend on the sense amplifier's (SA) process variation, and which match all the requirements for implementing PUFs described previously. %In our case, the dimension of our challenge input space. With our mechanism we can do many challenges on the same chip (one per row buffer)}
% With an Amnesic DRAM, we can do many challenges on the same chip (one per row buffer).
% 
% 
%%SA designs in which the restoration values are biased (like in the Figure~\ref{fig:process_variation}) work better as a PUF, since for the same challenge the same response will be produced. However, as can be observed from our evaluation in Section~\ref{sec:eval_randomnes}, there are some columns which do not produce consistent responses when the same challenge is applied. These values can hence be used as a source of randomness.
%%In SA's designs in which the restoration values are biased (cf.\ Figure~\ref{fig:process_variation}), the effects of process variation in the restoration values will manifest with a lower probability compared to non-biased designs.
%%In particular, SA's designs can bias the restored values either toward zero or one, skewing the distribution of the randomness introduced by process variation as a consequence. For instance, if the design is biased towards '0', e.g.\ the $+2\delta$ case in Figure~\ref{fig:process_variation}, a '1' due to process variation will manifest with a lower probability than a '0', since a bigger variation needs to occur for the restoration level to go below $0V$ than to stay above it.
%In particular, SA's designs can bias the restored values either toward zero or one, skewing the distribution of the randomness introduced by process variation as a consequence. For instance, if the design is biased towards '0', e.g.\ the common case in Figure~\ref{fig:process_variation}, a '1' due to process variation will manifest with a lower probability than a '0'.  In this example, this phenomenon happens because process variation can cause that a commom design behaves as $-2\delta$ design. %bigger variation needs to occur for the restoration level to go below $0V$ than to stay above it.

%In our evaluation (Section~\ref{sec:eval_randomnes}) we empirically demonstrate our observations. First, the DRAM chips that we tested have a biased design. Second, the probability of the process variation affecting the restoration process is usually low (~0.1\%), but enough to generate a set of unique and repeatable values that can be used as a UID for chip authentication. 

%Given these observations, the position of an SA within DRAM can be used as a PUF challenge, while the value read out from it after our \mechanism{} constitutes its response.

%%SA designs in which the restoration values are biased (like in the Figure~\ref{fig:process_variation}) work better as a PUF, since for the same challenge the same response will be produced. However, as can be observed from our evaluation in Section~\ref{sec:eval_randomnes}, there are some columns which do not produce consistent responses when the same challenge is applied. These values can hence be used as a source of randomness.



%%\todo{Mention the dimension of our challenge input space. With our mechanism we can do many challenges on the same chip (one per row buffer)}
%%are not very suitable for generating random numbers. However, it is a valid design to generate UIDs, as a few of these bits will show some unexpected behavior caused by process variation (see Section~\ref{sec:eval_randomnes}).

%%On another hand, this behavior is dictated by a design choice, and it could be easily changed. A secure chip based on our \mechanism{}, which aims to generate only random numbers even if the same challenge is applied, could be designed in such a way that the SA's restored values entirely depend on process variation in \mechanism{}s (see Section~\ref{sec:u-esa}).


%%On another hand, this behavior is dictated by a design choice, and it could be easily changed. A secure chip based on our \mechanism{}, which aims to generate only random numbers even if the same challenge is applied, could be designed in such a way that the SA's restored values totally depend on process variation in \mechanism{}s (see Section~\ref{sec:u-esa}).




%%\subsection{Bulk Initialization in Page Allocations}
%\subsection{Accelerating Page Allocations}
%\label{sec:initialization}
%\label{sec:pagealloc}
%%%%%%%%%%%%%%%%
%% Outline
%%%%%%%%%%%%%%%%
%%In the same way than Section~\ref*{sec:pagealloc}, we could generalize for any kind of memory initialization.
%%%%%%%%%%%%%%%%
%% Memset
%%%%%%%%%%%%%%%%



%%\subsubsection{Accelerating Page Allocations}

%%%%%%%%%%%%%%%%
%% Outline
%%%%%%%%%%%%%%%%

%%In this section we explain how to use the destructive activation for accelerate the zeroing in page allocations. This can be seen as a subset of Section~\ref{sec:initialization}, but  the difference with that Section is that here we can do lazy destruction easily using the page table.

%%%%%%%%%%%%%%%%
%% Accelerating Kernel Page Allocations
%%%%%%%%%%%%%%%%

%Virtual Memory (VM) is one of the most successful concepts in modern computer systems, and it is orchestrated by the Operating System (OS) and supported by hardware with the Memory Management Unit (MMU).  The OS has the responsibility of mapping the virtual addresses to physical addresses, manage page faults, etc.

%But the OS also have security responsibilities. It is critical to destroy previous data in new mapped pages, as otherwise, the information would leak between processes. The Linux kernel achieves this by zeroing the pages before the first access from the application. Zeroing pages can have a significant performance overhead, as we show in our evaluation (Section~\ref{sec:eval_pagealloc}).

%We can do memory zeroing efficiently with our D-TRAN implementation~\ref{sec:d-tran}. The method is as simple as emitting a \mechanism{} to the targeted row when a page initialization is performed.

%%Bulk initialization is the action of setting a large block of data to a particular value. 
%%This is a very common operation in modern systems,  especially to zero values~\cite{Jiang:2009,Yang2011,seshadri2013}. 


%Rowclone~\cite{seshadri2013} and Lisa-clone~\cite{Chang2016LISA} had proposed in-DRAM methods to initialize data to zero by copying a reserved row filled with zeros, to the destination row. The problem with these solutions is that they need to modify the internal architecture of DRAM and that the capacity of the DRAM is slightly reduced. Our \mechanism{} does not have the problems of these previous works, and the hardware overhead, energy, latency and the complexity are lower. This clearing operations on the kernel are some of the most critical in a modern system. %Previous works~\cite{seshadri2013,Chang2016LISA} on in-DRAM bulk initialization use kernel page clearing for evaluation.


%%\ipnote{Talk about that embedded systems, without virtual memory and without security concerns, disable memory clearing in new allocations to improve performance. So it is important for performance. }

%Although our unpredictable \mechanism{} (U-ESA and U-PLA) could also be used with the goal of destroying previous data, many libraries and applications still rely on that the pages allocated by the kernel are zeroed. They could be used only for systems that do not need zeroed pages in new allocations (like some embedded systems). %So, we consider only the D-TRAN implementation for better compatibility with current systems.

%%\subsection{Bulk Initialization}



%%%%%%%%%%%%%%%%
%% Outline
%%%%%%%%%%%%%%%%

%\paragraph{{\bf Lazy Amnesia}}
%\label{sec:lazy_zeroing}

%Our \mechanism{} has an additional advantage when used for clearing fresh mapped pages.

%By leveraging the existing virtual memory support, our \mechanism{} allows the lazy destruction of pages by using D-TRAN (or U-ESA if zeroing is not required). This means that the data does not need to be destroyed explicitly, but instead, it can be destroyed the first time the page is accessed, using a \mechanism{} instead of a regular activation.

%% TODO: improve this description
%The system support for implementing lazy amnesia is already present in modern operating systems. In page allocations, the newly allocated pages are mapped to a special page filled with zeros. Only on the first write, the OS physically allocates a new frame and it copies the content of the zero page to the new physical frame (this process is also known as copy-on-write, or CoW~\cite{gorman2004understanding}). By introducing our \mechanism{} with lazy amnesia, CoW is not needed anymore, as the page will be zeroed automatically when touched.

%Our lazy destroy mechanism virtually eliminates the latency of destroying data in page allocations.

%%% Why?
%% For security reasons, the linux kernel destroys the data of new allocated pages by zeroing their content. This has to be done each time a new anonymous page is allocated and touched for the first time.

%%In 64 bit systems, the page size is 8KB, that is the same size than a typical row in DRAM, which enables our mechanism to work at OS pages.
%%Despite many optimizations have been done to optimize the page zeroing, this could cause serious performance degradation in some demanding scenarios.
%%% CHECK: http://oss.sgi.com/projects/page_fault_performance/
%%% TODO: Userspace: Talk about mmap and brk.
%%The two main syscalls that the kernel provides to the user space for memory allocation are brk() and mmap().
%%% TODO: talk about randomization of memory in the kernel


%\subsection{Early Destruction of Data}
%\label{sec:early_destruction}

%Today's applications, especially web servers, web browsers, and word processors, do not immediately remove data from memory when it is no longer needed. Instead, the data is physically erased only when the memory is required for other uses. As a consequence, sensitive data could remain in memory for an indefinite amount of time, which augments the risk of exposure.


%Secure deallocation~\cite{chow2005shredding} is a technique that set the data to zero at the moment of deallocation, or as soon as the data is not needed anymore. This technique reduces the time that critical data is exposed to attacks. Vanish~\cite{Geambasu2009} propose a similar idea in which the old copies of data are self-destroyed after a specific amount of time.

%%Furthermore, use-after-free vulnerabilitiess~\cite{Caballero:2012, lee2015preventing} is one of the most common and critical attacks in software nowadays, especially in web browsers. This vulnerability is caused by a program operating in a dangling pointer. If the content of that pointer is physically destroyed at deallocation, we can prevent some of the attacks based on this vulnerability.

%Our \mechanism{} enables the implementation of the previous techniques with very low latency, energy, and area overhead (see Section~\ref{sec:eval_lat-ener-area}).

%%Reference~\cite{argyroudis2011}.

%%Use-after-free vulnerabilities~\cite{Xu2015}.


==> secureDeallocation.tex <==
%!TEX root =  main.tex
\section{Secure Deallocation}
\label{sec:secureDeallocation}

Today's applications and operating systems do not immediately delete data from memory when it is no longer needed. Instead, deallocated data could remain in physical memory for an indefinite amount of time until it is required again. This opens a window in which attackers can leak sensitive information by exploiting software vulnerabilities~\cite{Cowan:1998:SAA:1267549.1267554, smash}. Not deleting data on deallocation further enables attackers to perform attacks such as use-after-free exploitation~\cite{caballero2012undangle}. To counter these threats, Secure deallocation~\cite{chow2005shredding, Anikeev:2013, Sha2018, harrison2007protecting, geambasu2009vanish, Garfinkel:2004} sets the
data to zero at the moment of deallocation, or as soon as
the data is not needed anymore~\cite{geambasu2009vanish}. 

%\vspace{5pt}\noindent\textbf{Secure Deallocation and IoT} 
There are at least two major security challenges on IoT devices that could be mitigated with secure deallocation. First, the IoT devices that run programs with a high amount of lines of code (LoC)~\cite{LoC, TCROC} (e.g., high-end car's software is 100 million LoC~\cite{security_vehicles}) are difficult to debug and verify~\cite{hubert2005case}. Second, bare-metal systems rarely employ any security protection mechanisms (e.g., hard drive controllers~\cite{Zaddach:2013}) and their development assumptions (unrestricted access to memory), and constraints (runtime, energy, and memory) make applying protections challenging~\cite{Clements2017}. 

\vspace{5pt}\noindent\textbf{Low-cost Secure Deallocation} We propose to use \dtran{} for accelerating secure deallocation at low cost. Our mechanism outperforms the state-of-the-art in both performance and energy consumption as we show in Section~\ref{sec:eval_dealloc}, making it suitable for IoT devices. 

Enabling software support for secure deallocation requires the same changes as accessing Dataplant PUFs. These changes are described in  Section~\ref{sec:physicallyUnclonable}.
